Surface2Volume: Surface Segmentation Conforming Assemblable Volumetric Partition

Users frequently seek to fabricate objects whose outer surfaces consist of regions with different surface attributes, such as color or material. Manufacturing such objects in a single piece is often challenging or even impossible. The alternative is to partition them into single-attribute volumetric parts that can be fabricated separately and then assembled to form the target object. Facilitating this approach requires partitioning the input model into parts that conform to the surface segmentation and that can be moved apart with no collisions. We propose Surface2Volume, a partition algorithm capable of producing such assemblable parts, each of which is affiliated with a single attribute, the outer surface of whose assembly conforms to the input surface geometry and segmentation. In computing the partition we strictly enforce conformity with surface segmentation and assemblability, and optimize for ease of fabrication by minimizing part count, promoting part simplicity, and simplifying assembly sequencing. We note that computing the desired partition requires solving for three types of variables: per-part assembly trajectories, partition topology, i.e. the connectivity of the interface surfaces separating the different parts, and the geometry, or location, of these interfaces. We efficiently produce the desired partitions by addressing one type of variables at a time: first computing the assembly trajectories, then determining interface topology, and finally computing interface locations that allow parts assemblability. We algorithmically identify inputs that necessitate sequential assembly, and partition these inputs gradually by computing and disassembling a subset of assemblable parts at a time. We demonstrate our method....

==> 01_intro_old.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = 00_main.tex

\section{Introduction}
\label{sec:intro}
\cino{this is a comment from cino\\} 
\alla{this is a comment from alla\\}
\jaiko{this is a comment from marco\\}
\dany{this is a comment from daniela\\}

Thanks to the recent emergence of multi-material printers, geometric models can now be fabricated while accurately replicating both their geometry and appearance. Unfortunately, multi-material printing still exhibits severe limitations, and existing devices are either extremely expensive or produce rather low-quality results \cite{hergel14}. Independently of hardware limitations, an artist/designer is currently required to specify non-visible inner interfaces between different materials \cite{shmidt17, openfab}. We argue that many users are interested in how the physical object appears, while the separation between different materials within the solid is a manufacturing issue that an artist should not be called to solve.

To overcome these limitations, we propose an original algorithm that propagates color information from the boundary to the interior, without the need of any user intervention. Our propagation leads to a shape partitioning where each of the parts can be printed separately using a single color, and the set of all the parts can be eventually reassembled to form the target physical object with its expected appearance.

Notice that guaranteeing that the parts can be manually assembled without interference is surprisingly difficult. To simplify the problem, one may just thicken the surface towards the interior \cite{wang2013thickening} and propagate the surface colors along with the geometry. However, avoiding interference on concave areas is still an issue (see Fig. \ref{fig:no_solution}), and the resulting parts would be too fragile and difficult to be glued together due to their small contact areas. Furthermore, such a \emph{shell}-based approach would produce a separate part for each color-component on the surface, which may easily lead to unnecessarily many parts (Fig. \ref{fig:soccerball}) and to extremely small parts that can be hardly manipulated during the physical reassembly (e.g. the duck eyes in Fig. \ref{fig:duck}).

In contrast, our algorithm produces an assembleable set of bulk solid parts out of an input surface mesh with colored faces: starting from the assembled configuration, there exists a sequence of movements to \emph{extract} each of the parts along a specific direction without interference. Our calculation of the solid parts and their extraction directions depend on each other and, besides satisfying the extractability requirement, considers additional desirable characteristics to ensure practical usefulness: indeed, we wish to generate as few components as possible, and try to keep their size compatible with human manipulation. 



Although we cannot guarantee that our solution is optimal for any possible input configuration, we show that it is useful for practical cases.

Alternatively, one may try to apply Yao and colleagues work \cite{yao2017interactive} to generate bulk solid parts; however, this method was designed for decorative furniture joints modeled by few polygons covering large flat areas, and unfortunately appears to be inappropriate to handle even a moderately complex freeform model such as in Fig. \ref{fig:four_colors_sphere}.



We observe that modern filament deposition printers can be loaded with custom plastic filaments of any color, hence a possible approach would be to split the model into parts, each made of a single color, and then use such a printer fed with a properly-colored filament to fabricate each of the parts separately. 

In this paper, we introduce an original algorithm that produces an assemblable set of solid parts out of an input surface mesh with colored faces: each of the parts is made of a single color and, starting from the assembled configuration, there exists a sequence of movements to \emph{extract} each of the parts along a specific direction without interference. Our calculation of the solid parts and their extraction directions depend on each other and, besides satisfying the extractability requirement, considers additional desirable characteristics to ensure practical usefulness: indeed, we wish to generate as few components as possible, and try to keep their size compatible with human manipulation. Although we cannot guarantee that our solution is optimal for any possible input configuration, we show that it is useful for practical cases.

% THE FOLLOWING MIGHT BE MOVED TO THE CONCLUSIONS
%Furthermore, our tool makes the fabrication of multi-material objects cheaper and more accessible. When compared to multi-material printing, our approach has important advantages: the parts can be printed in parallel, which normally leads to a faster production, and the resulting quality in appearance can be sensibly higher (see Fig. \ref{fig:oozing}). One may argue that the need to assemble the parts represents a limitation, which is true. However, objects made of very different materials that cannot be managed by a single printer would need to be split in any case. Through our approach, dedicated devices can be used to produce the various parts depending on their specific needs (e.g. plastic-based FDM for the bulk structure, selective laser melting/sintering for metallic parts requiring high precision, high-quality CNC milling for parts that require a particular shininess).
%\begin{figure}
%	\includegraphics[draft,width=0.5\linewidth]{img/oozing.jpg}
%	\caption{The same object produced by dual-extrusion (a) and by parts (b). Note that the oozing effect in (a) can be mitigated by \cite{hergel14}, but in general it cannot be completely avoided.}
%	\label{fig:oozing}
%\end{figure}

